Privacy-Preserving Boosting in the Local Setting

In machine learning, boosting is one of the most popular methods that designed to combine multiple base learners to a superior one. The well-known Boosted Decision Tree classifier, has been widely adopted in many areas. In the big data era, the data held by individual and entities, like personal images, browsing history and census information, are more likely to contain sensitive information. The privacy concern raises when such data leaves the hand of the owners and be further explored or mined. Such privacy issue demands that the machine learning algorithm should be privacy aware. Recently, Local Differential Privacy is proposed as an effective privacy protection approach, which offers a strong guarantee to the data owners, as the data is perturbed before any further usage, and the true values never leave the hands of the owners. Thus the machine learning algorithm with the private data instances is of great value and importance. In this paper, we are interested in developing the privacy-preserving boosting algorithm that a data user is allowed to build a classifier without knowing or deriving the exact value of each data samples. Our experiments demonstrate the effectiveness of the proposed boosting algorithm and the high utility of the learned classifiers.

==> manuscript/sections/abstract.tex <==
\section{Abstract}
Ensemble learning is one of the most important components in machine learning area, which is designed to combine multiple base learners to a superior one. During the long development, boosting is one of the most popular methods and the boosted classifiers, like Boosted Decision Tree, have been widely adopted in multiple areas, such as text mining, financial and medical applications. In the big data era, data explosion  brings new challenges for the conventional machine learning algorithms. For instance, the data held by individual and entities, like personal images, browsing history and census information, are more likely to contain sensitive information. The privacy concern raises when such data leaves the hand of the owners and be further used in some computations. Such privacy issue prevents people contributing their data, and it brings the demand that the machine learning algorithm should be privacy aware and the privacy of the training samples should be protected. Recently, Local Differential Privacy is proposed as an effective privacy protection approach in the local setting, which states that a mechanism is local differentially private if it makes two data instances indistinguishable. LDP provides a strong privacy guarantee to the data owners, as the data is perturbed before any further usage, and the true values never leave the hands of the owners. Thus the development of machine learning algorithm with the private data instances is of great value and importance. In this paper, we are interested in developing the privacy-preserving boosting algorithm that a data user is allowed to build a classifier without knowing the exact value of each data samples or deriving any potential information. Our experiments demonstrate the effectiveness of the proposed boosting algorithm and its applicability to various types of classifiers.

==> manuscript/sections/encoder.tex <==
\section{DCAConv - Supervised Image Feature Extraction}

\begin{figure*}[ht!]
  \centering
    \includegraphics[width=0.95\textwidth]{./LDP_featureExtractor/extractor_1_2}
  \caption{DCAConv: Supervised Image Feature Extractor}
  \label{fig:extractor}
\end{figure*}
As analyzed in previous section, for both Naive Bayes and KNN classifiers, we show that the domain size of the input determines the utility gain regarding the perturbation of randomized response. For Naive Bayes, the utility can be measured by the variance of the estimated frequency. For KNN classifier, the utility is measured by the probability of preserving the true proximity between the testing data points and the perturbed training points. In terms of randomized response, it is readily to see that the utility gain is maximized when domain size $d=2$. However, the binary format limits the transited information, especially for the image data. On the other hand, increasing $d$ asks for more price to pay with respect to privacy. Thus the domain size $d$ is the very key factor for the trade-off between the utility and privacy. 


For image data, the naive way to protect the privacy is to apply randomized response to the pixel feature, nevertheless the utility is severely damaged due to the large domain size. Thus the challenge is to find a proper representation of the image data. On one hand, the representation should preserve as much information as possible; on the other hand, the domain size should provide a balance between the utility and privacy. The success of CNN\cite{krizhevsky2012imagenet} on image classification draws much attention in the last decade, which transforms the image into multiple level representations by extracting the abstract semantics. However, it is hard to apply randomized response to the CNN directly, the reason is that CNN usually needs continuous number in the data flow. Furthermore, it also relies on either Softmax or Sigmoid layer to determine the final output distribution, where the model is trained to optimize for specific loss functions. Inspired by PCANet\cite{chan2015pcanet}, we are interested in designing a mechanism to transform the image to a representation that has a scalable domain size. In the meanwhile, the domain size could be as small as possible to narrow the impact of randomized response in terms of utility. The outcome is DCAConv, as Fig.~\ref{fig:extractor} shows, which consists of the convolution layer, the binary quantization layer and the pooling layer. The convolution filter is computed using DCA and the generated discriminant components serve as the filter. The quantization layer converts the output of convolution operation to binary bits. Finally, images are represented with the mapping of the binary bits and passed through the pooling layer. The details are presented below:

\subsection{DCA Convolution Layer}
Suppose there are $N$ images $\{E_i\}^N_{i=1}$, each image has the same size $h \times w$, the patch size is $k_h \times k_w$, the number of filters in the $r$th convolution layer is $L_r$. $E_i$ is denoted as $[e_{i1}, e_{i2}, \dots , e_{i\widetilde{h}\widetilde{w}}]$, and $e_{ij}\in {\Bbb R}^{k_h\times k_w}$ denotes the $j$th vectorized patch in $E_i$, where $\widetilde{h} = (h-k_h+2z)/t+1, \widetilde{w} = (w-k_w+2z)/t+1$, and $t$ is the size of stride, $z$ is the the size of zero padding. Additionally, assuming there are $K$ classes, each image $E_i$ associates with a class label $y_i$ where $y_i\in \{C_{1}, C_{2}, \dots, C_{k}\}$, and each class $C_k$ contains $N_k$ images. For the first convolution layer, the overall patch mean $\mu$ and within class patch mean $\mu_k$ is calculated as below:
\begin{align}
  \mu & = \frac{\sum_{i=1}^N\sum_{j=1}^{\widetilde{h}\widetilde{w}} e_{ij}}{N} \\ 
  \mu_k & = \frac{\sum_{i\in C_k}^N\sum_{j=1}^{\widetilde{h}\widetilde{w}} e_{ij}}{N_k}
\end{align}
Then the between-class scatter matrix $S_B$, the within class scatter matrix $S_W$ and regularized scatter matrix are calculated as below:
\begin{align}
  S_B &= \sum^{K}_{k=1}N_k(\mu_k-\mu)(\mu_k-\mu)^T \\ 
  S_W &= \sum^{K}_{k=1} \sum_{i \in C_k} (E_i-\mu_k)(E_i-\mu_k)^T \\
  \bar{S}' &= S_{B}'+S_{W}'=S_{B}+\rho' \mathbb{I} + S_{W}+\rho \mathbb{I}
\end{align}
Once getting $S_W$ and $\bar{S}'$, DCA is performed over the patches and compute a set of discriminant components as the orthonormal filters, where:
\begin{equation}
(S_{W}')^{-1}\bar{S}' = U\Lambda U^T
\end{equation}
where $U$ holds the associated eigenvectors. The leading eigenvectors capture the main discriminant power of the mean-removed training patches. Then the first $L_1$ eigenvectors are taken as the orthonormal filters, where the $l$th filter is represented as $W^l_1\in {\Bbb R}^{k_h\times k_w}$, in the first convolution layer. 

Similar to CNN, multiple convolution layers could be stacked following the first layer, as Fig.~\ref{fig:extractor} shows. Given a second convolution layer as example, it repeats the similar procedure as in the first one. Given the $l_1$th filter in the first layer, for image $E_i$:
\begin{equation}
E_i^{l_1} = E_i * W^{l_1}_1, i = 1,2,\dots,N, l_1 = 1,2,\dots,L_1
\end{equation}

where $*$ denotes the 2D convolution. It could use zero padding on $E_i^{l_1}$ to make it has the same size as $E_i$. After that, the patch mean of $E_i^{l_1}$ is removed, then it performs DCA over the concatenated patches and computes the filters for the second convolution layer. Once DCA is finished, the first $L_2$ eigenvectors are taken as the filters, the $l$th filter in the second layer is represented as $W^l_2,W^l_2\in {\Bbb R}^{k_h\times k_w}$. For each $E_i^{l_1}$, there are $L_2$ filters to be convolved, as Fig.~\ref{fig:extractor} shows. 

\subsection{Binary Quantization}
After second convolution layer, there are $L_1\times L_2$ output in total, and they are converted to binary representation using the Heaviside step function $H(\cdot)$:
\begin{equation}
H(x) = 
\begin{cases}
    0, x \leq 0 \\
    1, x > 0   
\end{cases}
\end{equation}
where $x=E_i^{l_1}*W^{l_2}_2,l_1 = 1,2,\dots,L_1,l_2 = 1,2,\dots,L_2$.

\subsection{Mapping}
Once the output of the second convolution layer is converted to binary, for $E_i^{l_1}$, it obtains $\{H(E_i^{l_1}*W^{l_2}_2)\}_{l_2=1}^{L_2}$, which is a vector of $L_2$ binary bits. Since $E_i^{l_1}$ has the same size as $E_i$ with zero padding, for each pixel, the vector of $L_2$ binary bits is viewed as a decimal number of $L_2$ digits. It ``maps'' the output back into a single integer:
\begin{equation}
T_i^{l_1} = \sum^{L_2}_{l_2=1}2^{l_2-1}H(E_i^{l_1}*W^{l_2}_2)
\end{equation}

\subsection{Max Pooling}
The output of the binary quantization layer are $L_1$ ``images'' with each ``pixel'' of $L_2$ digits. To further reduce the size of the representation, for $T_i^{l_1}$, a max pooling layer is applied after the binary quantization layer.


\subsection{Perturbation}
The randomized response is applied to the output of the pooling layer, and the domain size $d$ is determined by $L_2$, where $d=2^{L_2}$. As we mentioned early, in DCA, the rank of the signal space is limited by the number of classes. More specially, $L_r \leq K$, where $L_r$ is the number of filters in $r$th convolution layer and $K$ is the number of classes. By employing DCA in the design, the domain of the final output is scalable, moreover, DCA also guarantees a high utility with a small number of components.
\iffalse
\subsubsection{Histogram Pooling}
Comparing to max pooling, histogram pooling provides augmented information within the pooling window. Rather than only taking the maximum value, a histogram of the decimal values in each window is computed and all histograms are concatenated into one vector, which is denoted as $hist(T_i)$. Then each $T_i$ represented as a block-wise histograms. 

For this histogram pooling, the $d$ in the randomized response is determined by the window size, where $d=p_1\times p_2$. It is readily to see that if the size of the pooling window is small, like $2\times 2$, the perturbation of the feature vector is small. Moreover, since the histogram provides more information than max pooling, the classification performance is expected to be better than max pooling method, and our experiments confirms this expectation.
\fi

==> manuscript/sections/introduction.tex <==
\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
\iffalse
\IEEEPARstart{M}{achine} learning as a service(MLaaS) has been growing rapidly as a cloud service. Amazon\cite{amazonAWS}, Google\cite{googleCloud} and Microsoft\cite{azureCloud} all offer such a platform for people to train and deploy a machine learning model on the cloud servers. During the training phase, the data owner who holds the dataset allows the platform API to access the data and then proceeds to train a machine learning model. During the testing phase, the data owner may evaluate the learned model with some unseen data. The MLaaS saves the hassles of deploying infrastructure and development environment for non-machine learning expertises. However, the privacy and confidentiality issue raises with the sensitive dataset. For instance, the hospital, who holds a set of X-ray images, wishes to train a model to help disease diagnosis; the authority, who holds the facial data of person of interest, wishes to train a model to help identify the PoI. Such medical and facial data certainly contains the sensitive information, where the content can’t leak to the MLaaS during the training and testing process.

Recently, studies on privacy preserving machine learning provides several solutions regarding MLaaS based on either Secure Multiparty Computation\cite{hesamifard2017privacy}\cite{mohassel2017secureml} or trusted processor, like Intel's SGX processor\cite{ohrimenko2016oblivious}\cite{hunt2018chiron}. Nevertheless, the former brings several orders of magnitude computation cost comparing to the plaintext data, and the latter needs to upgrade the hardware equipments. In contrast, Local Differential Privacy(LDP)\cite{duchi2013local}\cite{wang2017locally}\cite{bassily2017practical}\cite{cormode2018privacy} shows us another promising solution, which has been proposed to address the privacy preserving data collection problems. Regarding MLaaS, it allows the data owners randomly perturbing their inputs to provide plausible deniability of the data before revealing to the platform API. 

Randomized Response\cite{warner1965randomized} is a decades-old technique which designs for collecting sensitive survey in social science, and it\cite{wang2016private} has been proven that this technique satisfies $\epsilon$-LDP. However, a naive adoption of randomized response to the image data greatly hurts the utility of the underlying data because of too much perturbation regarding the pixel domain. Inspired by the randomized response and Convolutional Neural Network(CNN), we propose a light-weight privacy preserving feature extractor that satisfies $\epsilon$-LDP. We also analyze the utility of the extracted feature in terms of the Euclidean distance and demonstrate the utility through multiple classification algorithms, like linearSVM, KNN and Random Forest, and the result shows that the proposed mechanism maintains a good utility of the underlying data.

\begin{itemize}
\item We propose a privacy preserving image feature extractor that satisfies $\epsilon$-LDP. To the best of our knowledge, most LDP-based work focus on the frequency estimation of the categorical data, and we are the first to develop the local differentially private feature extractor for image data. Moreover, we analyze the Euclidean distance between the perturbed data points after the perturbation, which shows that the exacted feature could maintain a high utility regarding the distance-based machine learning algorithm.  
\item The proposed light-weighed feature extractor is inspired by CNN, but has less computation cost. Instead of performing the forward and backward propagation in CNN, our feature extractor only requires one forward computation, which greatly reduce the computation. 
\item We have perform extensive experiments regarding multiple datasets, like MNIST and CIFAR dataset. Since the state-of-art accuracy of image recognition is achieved by CNN-based classifiers, we also compare with the feature extracted by different type of CNN classifiers and show that the proposed work achieves a compatible accuracy.  
\end{itemize}
\fi

Image data has been greatly produced and shared in our daily life, and the usage of image data has been demonstrated through various applications, like preference analysis and advertising\cite{leon2012johnny}, medical \cite{xia2016privacy} and traffic\cite{chan2008privacy} analysis. Lately, image data becomes greatly important in social utility\cite{lepinski2016privacy} as well, like emergency response. For example, in the Boston Marathon bombing, the authorities spent lots of effort to gather onsite photos from people in that area, and pore through thousands of photos to search for the suspects. However, the privacy concern comes to be the biggest obstacle that prevents people sharing this information, since the image may reveal where they are and what they are doing. Thus, exploring the privacy preserving machine learning technique with regard to image data becomes paramount importance.

\iffalse
In addition, the modern deep learning models show a great success of machine learning tasks with respect to image data, like Fully Convolutional Neural Network\cite{Long_2015_CVPR} and ResNet\cite{He_2016_CVPR}.

The privacy preserving image classification problem has been investigated through some cryptography-based methods. Erkin et al.\cite{erkin2009privacy} applies Secure Multiparty Computation (SMC) in a privacy-enhanced face recognition system. With their solution, one party who holds a facial image and another party who holds the facial database jointly run the standard Eigenface recognition algorithm. It guarantees that the first party only learns whether the held facial image is in the database, while the second party would not learn the input. A following work\cite{sadeghi2009efficient} improves the efficiency by combining the homomorphic encryption and garbled circuits. As the previous work requires several orders of magnitude computation cost comparing to the plaintext data due to the cryptography technique, 

\begin{figure}
  \centering
    \includegraphics[width=0.5\textwidth]{./researchProblem/problem}
  \caption{Each image $X_i$ is perturbed by the same $\epsilon$-LDP mechanism. The data user only receives the perturbed data $X_i'$ and proceeds with machine learning tasks with these data as input.}
  \label{fig:problem}
\end{figure}

\fi

In this paper, we study an image classification problem, in which there are two parties\cite{kairouz2014extremal}, the image owners, who hold a set of images; the untrustworthy data user, who would like to fit a machine learning model regarding these images. As an example, in the Marathon bombing case, the authorities serves as the data user, who asks for the onsite images to search for the suspects, and the people that provided the images serve as the data owner, who wishes to support the investigation while preserving the privacy. During the last decade, Differential Privacy \cite{Dwork2006DP} is one of the most popular schemes for privacy protection, which prevents the inference about individuals from participation of computation. It defines a mechanism that the computation of the data is robust to any change of any individual sample by introducing uncertainty into the algorithm. Recently, Local Differential Privacy(LDP)\cite{duchi2013local}\cite{wang2017locally} extends the technique into a local setting, which provides a stronger privacy protection that allows data owners to perturb their input before releasing.


Differentially private machine learning in the local setting has been rarely studied. Recently, \cite{nguyen2016collecting} and \cite{pihur2018differentially} investigate the privacy-preserving distributed machine learning, in both work, the data owners interactively work with the data user to learn the model. Unlike these previous work, a ``non-interactive'' manner draws much of our interest that the data owners only perturb once and then share the data with the data user. Comparing to the interactive setting, the non-interactive way is more scalable and needs less communication cost. Randomized response\cite{warner1965randomized} is proposed to provide the plausible deniability for individuals responding to sensitive surveys. It has been proved that this mechanism satisfies $\epsilon$-LDP and is universally optimal for mutual information optimization problem\cite{kairouz2014extremal}, which provides a solid foundation for its usage in the area of machine learning. In this paper, we are interested in adopting randomized response to locally perturb the input and fit the count-based and distance-based machine learning models with such input. Specifically, we study the utility and privacy trade-off with respect to the Naive Bayes and KNN classifiers and show how the model utility is affected by the privacy parameters. Furthermore, in terms of image classification, we propose the DCAConv, a supervised image feature extractor, that improves the utility under the $\epsilon$-LDP. 


Overall, the contributions of our work are three folds:

\begin{itemize}
\item We propose to use the LDP in the privacy preserving image classification problem. To the best of our knowledge, most LDP-based work focus on the frequency estimation of the categorical data, and we are the first to investigate the privacy preserving mechanism to fit the image data in the classification problem.
\item We analyze the utility and privacy trade-off regarding count-based and distance-based machine learning models, i.e. Naive Bayes and KNN classifiers. As a result, we show how the model utility is affected by the privacy parameters. 
\item We develop the DCAConv, a supervised image feature extractor, which represents the image with a scalable domain size. DCAConv is evaluated in terms of image classification through multiple benchmark datasets, like texture and facial datasets. The results confirm that DCAConv could maintain a high data utility while preserving the privacy.
\end{itemize}

The rest of paper is organized as follow. The preliminary is in Section II. The problem definition and proposed solution is introduced in Section III. We describe DCAConv, the supervised image feature extractor in Section IV. The experiment and evaluation is in Section V. The related work is presented in Section VI. Section VII presents the conclusion.
